TrustRAG: Enhancing Robustness and Trustworthiness in Retrieval-Augmented Generation

Retrieval-Augmented Generation (RAG) enhances large language models (LLMs) by integrating external knowledge sources, enabling more accurate and contextually relevant responses tailored to user queries. These systems, however, remain susceptible to corpus poisoning attacks, which can severely impair the performance of LLMs. To address this challenge, we propose TrustRAG, a robust framework that systematically filters malicious and irrelevant content before it is retrieved for generation. Our approach employs a two-stage defense mechanism. The first stage implements a cluster filtering strategy to detect potential attack patterns. The second stage employs a self-assessment process that harnesses the internal capabilities of LLMs to detect malicious documents and resolve inconsistencies. TrustRAG provides a plug-and-play, training-free module that integrates seamlessly with any open- or closed-source language model. Extensive experiments demonstrate that TrustRAG delivers substantial improvements in retrieval accuracy, efficiency, and attack resistance.

==> table/algorithm.tex <==
% \begin{algorithm*}[t]
% \caption{TrustRAG}
% \label{alg:method_with_kmeans}
% \begin{algorithmic}[1]
% \Require Query $q$, Retrieved documents $E_{\text{ori}} = [e_1, \ldots, e_n]$, LLM $\mathcal{M}$, Prompts $p_{\text{gen}}$, $p_{\text{con}}$, $p_{\text{ans}}$
% \Ensure Robust and trustworthy response $A$

% \Comment{\textbf{Stage 1: Clean Retrieval}}
% \State Perform K-Means filtering on $E_{\text{ori}}$:
% \begin{enumerate}[label*=\arabic*)]
%     \item Remove documents that are highly redundant or suspicious using similarity metrics and $n$-gram repetition.
%     \item Update the document set $E$ with the filtered subset.
% \end{enumerate}
% \State \textbf{Output:} Filtered external documents $E_{\text{filter}}$

% \Comment{\textbf{Stage 2: Knowledge Integration and Answer Generation}}
% \State Generate internal knowledge: $I \gets \mathcal{M}(p_{\text{gen}}, q)$
% \State Combine external and internal documents: $E_{\text{combined}} \gets E_{\text{filter}} \oplus I$
% \State Consolidate knowledge: $D_{\text{new}} \gets \mathcal{M}(p_{\text{con}}, q, E_{\text{combined}})$
% \State Generate final answer: $A \gets \mathcal{M}(p_{\text{ans}}, q, D_{\text{new}})$

% \State \Return $A$
% \end{algorithmic}
% \end{algorithm*}


==> table/closed_source_model.tex <==

\begin{table*}[ht]
\centering
\footnotesize
    \caption{This table presents the performance of defense frameworks applied to GPT$_{\text{4o}}$ integrated with RAG
systems against PoisonedRAG with different poison rates. The best performance of each model is highlighted in \textbf{bold}.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llcccccc}\toprule
Dataset & Defense & Poison-(100\%) & Poison-(80\%) & Poison-(60\%) & Poison-(40\%) & Poison-(20\%) & Poison-(0\%) \\
 & & \textbf{ACC} $\uparrow$ / \textbf{ASR} $\downarrow$ & \textbf{ACC} $\uparrow$ / \textbf{ASR} $\downarrow$ & \textbf{ACC} $\uparrow$ / \textbf{ASR} $\downarrow$ & \textbf{ACC} $\uparrow$ / \textbf{ASR} $\downarrow$ & \textbf{ACC} $\uparrow$ / \textbf{ASR} $\downarrow$ & \textbf{ACC} $\uparrow$  \\
\midrule \noalign{\smallskip}

%--------------------------------------
\multirow{5}{*}{NQ}
& Vanilla RAG& $20.0 / 80.0$ & $32.0 / 69.0$  &  $37.0 / 60.0$ & $49.0 / 49.0$ & $56.0 / 39.0$ & $76.0 $ \\
& RobustRAG$_{\text{Keyword}}$ & $1.0 / 61.0$ & $8.0 / 57.0$ & $20.0 / 58.0$ & $32.0 / 36.0$ & $39.0 / 28.0$ & $45.0 $ \\
& InstructRAG$_{\text{ICL}}$ & $13.0/83.0$ & $21.0/74.0$ & $27.0/65.0$ & $37.0/55.0$ & $53.0/39.0$ & $79.0$ \\
& ASTUTE RAG & $76.0 / 24.0$ & $76.0 / 21.0$  & $76.0 / 20.0$ & $78.0 / 16.0$ & $82.0 / 6.0$ & $81.0 $ \\
& TrustRAG$_{\text{stage 1}}$ & $79.0 / 6.0$ &  $65.0 / 15.0$ & $75.0 / 3.0$ & $73.0 / 3.0$ &$57.0 / 35.0$ &$76.0 $\\
& TrustRAG$_{\text{stage 1\&2}}$ & $\mathbf{81.0} / \mathbf{1.0}$ & $\mathbf{82.0} / \mathbf{3.0}$ & $\mathbf{80.0} / \mathbf{1.0}$ & $\mathbf{84.0 / 1.0}$  & $\mathbf{83.0}/ \mathbf{4.0}$ & $\mathbf{84.0}$ \\



\noalign{\smallskip} \hdashline \noalign{\smallskip}
\multirow{5}{*}{MS-MARCO}
& Vanilla RAG& $29.0 / 66.0$ & $43.0 / 49.0$ & $51.0 / 40.0$ & $59.0 / 35.0$ & $67.0 / 24.0$ & $81.0 $ \\
& RobustRAG$_{\text{Keyword}}$ & $2.0 / 63.0$ & $17.0 / 52.0$ & $23.0 / 48.0$ & $41.0 / 33.0$ & $50.0 / 22.0$ & $56.0 $ \\
& InstructRAG & $15.0/81.0$ & $31.0/64.0$ & $39.0/54.0$ & $47.0/45.0$ & $59.0/35.0$ & $81.0$ \\
& ASTUTE RAG & $67.0 / 24.0$ & $67.0 / 21.0$ & $72.0 / 17.0$ & $74.0 / 16.0$ & $77.0 / 13.0$ & $85.0 $ \\
& TrustRAG$_{\text{stage 1}}$ & $88.0 / 4.0 $& $76.0 / 11.0$ & $84.0 / \mathbf{2.0}$ & $84.0 / \mathbf{4.0}$ & $62.0 / 24.0$ & $77.0 $ \\
& TrustRAG$_{\text{stage 1\&2}}$ & $\mathbf{90.0} / \mathbf{2.0}$ & $\mathbf{90.0} / \mathbf{2.0}$ & $\mathbf{90.0} / 5.0$ & $\mathbf{87.0}/\mathbf{4.0}$  & $\mathbf{86.0} / \mathbf{8.0}$ & $\mathbf{89.0}$ \\

\noalign{\smallskip} \hdashline \noalign{\smallskip}
\multirow{5}{*}{HotpotQA}
& Vanilla RAG& $8.0 / 92.0$ & $33.0 / 67.0$ & $31.0 / 69.0$ & $48.0 / 52.0$  & $52.0 / 48.0$ & $82.0 $ \\
& RobustRAG$_{\text{Keyword}}$ & $5.0 / 76.0$ & $18.0 / 74.0$ & $20.0 / 61.0$ & $41.0 / 43.0$ & $51.0 / 27.0$ & $54.0 $ \\
& InstructRAG$_{\text{ICL}}$ & $1.0/98.0$ & $9.0/90.0$ & $19.0/79.0$ & $27.0/71.0$ & $33.0/63.0$ & $\mathbf{86.0}$ \\
& ASTUTE RAG & $66.0 / 35.0$ & $67.0 / 33.0$ & $74.0 / 25.0$ & $76.0 / 24.0$ & $78.0 / 22.0$ & $80.0 $ \\
& TrustRAG$_{\text{stage 1}}$ & $\mathbf{82.0} / 5.0$ & $77.0 / 12.0$ & $85.0 / 5.0$ & $\mathbf{81.0} / 10.0$ & $54.0/ 46.0$ & $76.0 $ \\
& TrustRAG$_{\text{stage 1\&2}}$ & $81.0 / \mathbf{3.0}$ & $\mathbf{84.0} / \mathbf{1.0}$ & $\mathbf{81.0} / \mathbf{3.0}$ & $\mathbf{81.0} / \mathbf{4.0}$ & $\mathbf{84.0} / \mathbf{6.0}$ & $84.0$ \\

\bottomrule
\label{table: closed_source_model}
\end{tabular}}
\end{table*}
